Path-Tree Optimization in Discrete Partially Observable Environments using Rapidly-Exploring Belief-Space Graphs

Robots often need to solve path planning problems where essential and discrete aspects of the environment are partially observable. This introduces a multi-modality, where the robot must be able to observe and infer the state of its environment. To tackle this problem, we introduce the Path-Tree Optimization (PTO) algorithm which plans a path-tree in belief-space. A path-tree is a tree-like motion with branching points where the robot receives an observation leading to a belief-state update. The robot takes different branches depending on the observation received. The algorithm has three main steps. First, a rapidly-exploring random graph (RRG) on the state space is grown. Second, the RRG is expanded to a belief-space graph by querying the observation model. In a third step, dynamic programming is performed on the belief-space graph to extract a path-tree. The resulting path-tree combines exploration with exploitation i.e. it balances the need for gaining knowledge about the environment with the need for reaching the goal. We demonstrate the algorithm capabilities on navigation and mobile manipulation tasks, and show its advantage over a baseline using a task and motion planning approach (TAMP) both in terms of optimality and runtime.

==> src/02_b_related_work.tex <==
% POMDP... general, but intractable esp. for continuous state action space.
% Assumptions to to make it tractable for robotic systems:
%% 1/ discretize, state / action space
%[1][2]
%% (replace PO, information gathering need [o7][o8][o9])

%% 2/ assume more structure of the belief state: gaussian, localization, BRP
%[3][4][o5][o6][o10][o11][o12]

%% 3/ discrete observation, mode switches, multi-modality: contingent [o13], 
%
%--------------------------------------------------------------------%
% Sampling-based multi-modal planning, multimodal for different tasks
% similarity in how a shared sampling based structure is re-used across modes to improve the sample-efficiency
% [5][6][7]

%--------------------------------------------------------------------%
% multi-hypo-these belief space planning for space exploration / SLAM.  

% general pomdp
Motion Planning under partial observability, can be generally framed as Partially Observable Markov Decision Processes (POMDP). However, solving POMDPs~\cite{kaelbling1998planning} is often intractable, such that computing policies (mapping belief-state to actions) is often restricted to simple, low-dimensional domains~\cite{grady2013combining}, or to abstracted versions of the initial problems~\cite{wang2018bounded}. 

% gaussian
Tackling real-world partially observable motion-planning problems, typically involves sacrificing some generality to gain improve scalability. One common approach for navigation tasks consists in modeling  the belief states as Gaussians (e.g. often to model localization uncertainty)
%traj%
and to plan paths in belief-space (in opposition to reactive policies). Under those working hypotheses, several generalization of classical sampling based planner~\cite{kavraki1996probabilistic}\cite{lavalle1998rapidly} have been developed. In particular, our approach has similarities with \cite{prentice2010belief}\cite{zheng2021belief}\cite{bry2011rapidly}, which plans in belief space on a graph-based transition system in a sampling based fashion. However, we focus on problem where the partial observability is not uni-modal and continuous (like a Gaussian) but discrete and multi-modal and where efficient planning requires planning different contingencies (in opposition to a sequential path). 
%contingencies%

In the field of object manipulation planning \cite{pall2018contingent} also presents similarities to our approach. It finds contingency plans based on contact sensing. Contacts help to reduce the uncertainty over the relative position of the object to manipulate. It is a continuous uncertainty, while this paper focuses on the environment multi-modality. In addition, we aim for optimality whereas \cite{pall2018contingent} aims only for feasible policies. 

%belief space planning, multi-modality -> path aspect, joint pace
%synthesis work?
%Mixed RRT?

%Another direction of work, 

%To make a partially observable robotic planning problem tractable, additional assumptions about the problem structure, are often made.

%One typical way is to to reduce the problem dimensionality, by introducing symbolic abstractions, or by discretizing the state and/or action spaces. For example [] synthesises POMDPs policies for problems similar to our experiments (e.g. fetch a target object which location is unknown). However, the initial action space simplification lead to plans are high-level and aren't optimal paths. % put more about POMDPs?

%In contrast, our approach aims at planning optimal paths, potentially high dimensional space. To avoid the curse of dimensionality, a simplified belief-dynamic is assumed at planning time (non stochasticity of the observations, countable number of belief states). We discuss in section XX how the offline computations can be re-used at execution time for online re-planning.

%Another class of method assumes gaussian belief-states, often to tackle localization uncertainty [5][6][11]. Similar to those approaches, we plan in belief-space on a transition system grown in a sampling-based fashion. However, we focus on problem where the partial observability is not uni-modal and continuous (like a Gaussian) but discrete and multi-modal and where efficient planning requires planning different contingencies.

%This combination of multi-modality and sampling-based motion planning also shows similarities TAMP sampling based methods that plan paths spanning across multiple manifolds representing multiple modes.


==> src/02_c_related_work.tex <==
%A rich body of work has focused..

Many adaptations of classical sampling-based planners~\cite{lavalle1998rapidly, kavraki1996probabilistic} have been developed for POMDP-like problems.

% gaussian + continuous observations
One group of algorithms assume continuous observations and gaussian beliefs-states (often to tackle the localization uncertainty). Roadmap-based approaches \cite{prentice2010belief}\cite{bry2011rapidly}\cite{leahy2019control}\cite{zheng2021belief} sample a roadmap in a sampling-based fashion, and belief-space planning is achieved on this transition system. An observation model is used to infer the belief-state dynamic.

The main idea that we share with those approaches is the roadmap structure grown in a sampling based fasion. The main difference lies in the kind of partial observability that we model (discrete and multi-modal vs. gaussian and unimodal) and in the nature of the solution (sequential plan vs. reactive path-trees).


% discrete observations
Another group of algorithms performs contingent planning based on discrete observations. In the field of object manipulation planning \cite{pall2018contingent}. It finds contingency plans based on contact sensing. Contacts help to reduce the uncertainty over the relative position of the object to manipulate. It is a continuous uncertainty, while this paper focuses on the environment multi-modality. In addition, we aim for optimality whereas \cite{pall2018contingent} aims only for feasible policies. 
% reuse the sampling data-structure across mode for efficiency

% multi-modal
%% state estimation
%% TAMP sampling-based

% use case: mapping
%Another closely related line of work plans paths which maximize the information gathered along the path \cite{hollinger2014sampling} \cite{levine2010information} \cite{dang2020graph}. Like the previously mentioned work, a graph or tree is grown in a sampling-based fashion. However, instead of planning in belief-space, those approaches determine the optimal traversal w.r.t. an information objective, e.g. volumetric gain for the use case of mapping in \cite{dang2020graph}.

% use case: monitoring
%Another direction of research uses sampling-based methods for planning problems where the goal is expressed as a temporal logic specification \cite{karaman2009sampling} \cite{leahy2019control} \cite{vasile2020reactive}. Similarly to the method of this paper, the output solution of the planning problem is more general than a sequence of states. In \cite{karaman2009sampling} \cite{vasile2020reactive}, the solutions are cyclic infinite paths. 

% extension of the GDTL
% transition system in belief space
% localization 
% feedback controller
% 2 stages
% synthesize control policy
% goal condition specifies constraints about the localization uncertainty
% uncertainty seen as noise
% FIRM Feedback Information Roadmap
% policy that satisfies the goal with a high enough satisfaction probability
% with the crucial difference that the uncertainty is continuous and over the robot localization and assumed to be gaussian. On the other hand our 
% belief update with kalman filter

%It  but can take the form of cycles.
%%XX is the closest related work

% connect to use case.. monitoring


%In particular xy show similarities with our approach in that the combine a first step of graph growing in belief space and second step of path extraction.

%Like our approach 

%path planning in the presence of goal uncertainty; 
%Belief space path planning
%Non-linear policies RRG
%View planning
%POMDP Navigation

==> src/05_experiments_before.tex <==

The path-tree optimization algorithm is implemented in the Rust programming language \cite{matsakis2014rust}. The application layer is implemented in C++ using MoveIt \cite{coleman2014reducing}. The source code and a supplementary video are available for reference \footnotemark \footnotetext{\href{https://github.com/cambyse/po-rrt}{https://github.com/cambyse/po-rrt}}.

\subsection{Mobile robot navigation} \label{experiment:navigation}
We consider two planning problems similar to the initial example introduced in Fig.~\ref{fig:intro}. The robot is the Kobuki platform. The robot has to reach a predefined goal region, but at planning time, it doesn't know which doors are open. The observation model simulates that the sensor mounted on the Kobuki and the perception pipeline allow the robot to know if a door is open once the robot is close to a door (less than 1.5 m) and has a non-occluded line of sight to the door. We plan for the two-dimensional position of the robot.

The first problem, called problem-A (Fig.~\ref{fig:problem_a_influence_belief_states}) has two uncertain doors. The second problem, called problem-B (Fig.~\ref{fig:problem_b}) is more complex, the map is larger, there are four doors, and more obstacles.
\begin{figure}[h]
	\begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_0p7.png}
		 \caption{Path-tree obtained with a high likelihood that doors are open (80\%). The path-tree has 2 branching points corresponding to the observation of the 2 doors.}
         \label{fig:0p7_belief_state}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_0p25.png}
		\caption{Path-tree obtained with 50\% of likelihood that doors are open: It is not advantageous to attempt the direct way through the doors.}
    \label{fig:0p25_belief_state}
	\end{subfigure}
	\caption{Problem-A: The robot has to reach the green region on the right.}
	\label{fig:problem_a_influence_belief_states}
\end{figure}

\begin{figure}[h]
	\begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_execution_0.png}
         \label{fig:problem_a_world_0}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_execution_1.png}
    \label{fig:problem_a_world_1}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_execution_2.png}
         \label{fig:problem_a_world_2}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.485\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_0/path_tree_execution_3.png}
         \label{fig:problem_a_world_3}
	\end{subfigure}\hfill
	\caption{Path-tree execution in several worlds: The robot potentially has to backtrack if it ends up in a dead-end after observing the second door.}
	\label{fig:problem_a_path_executions}
\end{figure}

Fig.~\ref{fig:0p7_belief_state} shows the path-tree obtained when the initial belief-state corresponds to a high likelihood that each door is opened (80\%). In that case, it is advantageous to attempt the direct path through the doors. The path-tree has two branching points  corresponding to the observations of the two doors. Fig.~\ref{fig:problem_a_path_executions} shows the execution of the path-tree in each possible world. In the best case, the two doors are open and the robot reaches the goal directly. In the worst-case, the robot ends up in a dead-end and has to backtrack after observing that the second door is closed.

In this example, we see the strong influence of the initial belief-state on the topology of the path-tree: Fig.~\ref{fig:0p25_belief_state} shows the path-tree obtained with an initial belief-state corresponding to a probability of only 50\% that the doors are open. In that case, it is not worthy to attempt the way through the doors, the planned path takes the longer, but sure way to the goal. The path-tree boils down to a sequential path without observing branching points. 
%Figure shows a trajectory-tree.
% influence of the belief state. Similar to TAMP, discrete decisions.

%\begin{figure}[h]
\setlength{\columnsep}{6pt}%
\begin{wrapfigure}{l}{0.3\textwidth}
\includegraphics[width=0.3\textwidth]{drawings/3_navigation/map_4/path_tree.png}
\caption{Path-tree for Problem-B: The map has four doors leading to a more complex path-tree.}
\label{fig:problem_b}
\end{wrapfigure}
%\end{figure}

%scalability
Fig.~\ref{fig:problem_b} shows the path-tree obtained for the problem-B, and Fig.~\ref{fig:problem_b_path_executions} shows its execution in a subset of the possible worlds. The higher number of doors leads to a path-tree which is much more complex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
	\begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_0.png}
         \label{fig:problem_b_world_0}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_1.png}
    \label{fig:problem_b_world_1}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_2.png}
         \label{fig:problem_b_world_2}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_3.png}
         \label{fig:problem_b_world_3}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_4.png}
         \label{fig:problem_b_world_4}
	\end{subfigure}\hfill	
	\begin{subfigure}[b]{0.33\linewidth}
		\centering
		\includegraphics[width=\textwidth]{drawings/3_navigation/map_4/path_tree_5.png}
         \label{fig:problem_b_world_5}
	\end{subfigure}\hfill
	\caption{Path-tree execution: The robot explores the doors on the left of the map. It potentially has to back-track and take the long route if it is blocked.}
	\label{fig:problem_b_path_executions}
\end{figure}

Table~\ref{tab:planning_times_navigation}, gives the expected costs to goal, and the planning times obtained when running the planning algorithm 20 times. Each problem is solved using 2 different strategies for the RRG sampling: In the initial variation, the RRG sampling is stopped as soon as completeness is guaranteed (see \ref{section:rapidly-exploring-random-graph}), and the second variations (A$^\prime$ and B$^\prime$) use a minimum number of 5000 iterations to obtain a more qualitative path-tree.

\begin{table}
\begin{center}
\footnotesize
\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{|l||l|l|l|l|l||l|l|}
\hline
                             & \thead{\# of\\ iter}  & \thead{random\\graph\\creation} & \thead{belief-\\space\\expansion} & \thead{policy\\ extraction} & \thead{partial\\shortcut} & \thead{path\\cost} & \thead{total\\planning\\time (ms)} \\ \hline
A & \thead{433\\(107)} & \thead{0.72\\(0.44)} & \thead{0.98\\(0.51)} & \thead{0.54\\(0.27)} & \thead{0.49\\(0.28)} & \thead{18.6\\(0.37)} & \thead{2.78\\(1.4)} \\ \hline
A$^{\prime}$ & \thead{5000\\(0)} & \thead{30.9\\(3.7)} & \thead{29.1\\(2.80)} & \thead{16.7\\(1.1)} & \thead{0.31\\(0.05)} & \thead{18.17\\(0.1)} & \thead{77.1\\(6.02)} \\ \hline
B & \thead{3956\\(626)} & \thead{44.7\\(14.3)} & \thead{345\\(102)} & \thead{173\\(60.8)} & \thead{3.25\\(1.07)} & \thead{45.1\\(1.74)} & \thead{567\\(174)} \\ \hline
B$^{\prime}$ & \thead{5000\\(0)} & \thead{61.5\\(6.49)} & \thead{538\\(32)} & \thead{270\\(22.9)} & \thead{2.95\\(0.38)} & \thead{43.9\\(1.25)} & \thead{873\\(47.1)} \\ \hline
\end{tabular}
\end{center}
\caption{Planning time and expected cost: The mean value is given first. The standard-deviation is in parentheses. Times are in milliseconds.}
\label{tab:planning_times_navigation}
\end{table}

Generally, the algorithm is fast, and takes less than 1~second even for the most complex map. The step taking the longest time is the graph expansion to belief-space (see \ref{section:graph_expansion_belief_space}). The reason is that the number of belief-states grows quickly when the number of doors increases, and the observation model is queried for each belief-space node.

Increasing the number of iterations results in smaller expected costs of the path-tree, at the expense of the overall runtime. In practice, the final refinement step (see \ref{section:refinement}) leads to path-trees that are already near-optimal even without a very high number of iterations, such that it is an efficient strategy to keep a small number of minimal iterations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robot arm object fetching} \label{experiment:mobile_manipulation}
% influence of the number of iterations on the quality?
% Runtime per algorithm stage, cost in joint space
% picture sensor field of view etc?
Our next scenario is a Panda arm robot mounted on a mobile base. We introduce two examples, where the task is to pick-up an object which is at an unknown location (see problem-A on Fig.~\ref{fig:arm_example_1} and problem-B on Fig.~\ref{fig:arm_example_2}). The robot has prior knowledge of several potential locations, but the actual location is unknown at planning time. 

\begin{figure}[!htb]
 \center{\includegraphics[width=0.45\textwidth]{drawings/2_arm/example_1.png}}
 \caption{Problem-A: The robot has to pick the green block. The block location is unknown, it may be on each one of the three shelves.}
 \label{fig:arm_example_1}
\end{figure}

The observation model simulates that a sensor is placed on the robot gripper and that the perception pipeline detects the block when it is within the sensor field of view (60$^{\circ}$), at a distance less than 2 meters from the sensor, and not occluded by other objects (e.g. the walls).

\begin{figure}[!htb]
 \center{\includegraphics[width=0.45\textwidth]{drawings/2_arm/example_2.png}}
 \caption{Problem-B: The block might be on two different shelves. The opening between the two doors potentially allows the robot to observe the shelves without entering the rooms.}
 \label{fig:arm_example_2}
\end{figure}

Planning is performed in joint space with 9 degrees of freedom (2 for the base, and 7 for the robot arm). 
Fig.~\ref{fig:example_1_path_tree} shows the trajectory of the robot base. There are two observation branching points corresponding to the observations of the two shelves.
%
\begin{figure}[!htb]

 \center{\includegraphics[width=0.45\textwidth]{drawings/2_arm/example_1_path_tree.png}}
 \caption{Path-tree for Problem-A: The path tree first moves towards the shelf\_0 to reach the first viewpoint. If the object is on the shelf\_0, the green path is executed. Otherwise the robot moves towards the second viewpoint.}
 \label{fig:example_1_path_tree}
\end{figure}
%
Fig.~\ref{fig:example_2_view_point} shows the robot configuration at the branching point of the path-tree. The opening in the wall allows the robot to take a look at the shelf.

\begin{figure}[!htb]
 \center{\includegraphics[width=0.45\textwidth]{drawings/2_arm/example_2_viewpoint.png}}
 \caption{Path-tree for Example-B: A first common branch of the path-tree leads the robot to an observation point through the opening. Depending on the observation, the robot will execute the green or the magenta path.}
 \label{fig:example_2_view_point}
\end{figure}

We report in Table~\ref{tab:planning_times} on the average path-tree cost and planning time obtained over 100 planning queries. 
%
%%%%
\begin{table}
\begin{center}
\footnotesize
\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{|l||l|l|l|l|l||l|l|}
\hline
                             & \thead{\# of\\ iter}  & \thead{random\\graph\\creation} & \thead{belief-\\space\\expansion} & \thead{policy\\ extraction} & \thead{partial\\shortcut} & \thead{path\\cost} & \thead{total\\planning\\time (s)} \\ \hline
A & \thead{10521\\(16481)} & \thead{5.86\\(14.7)} & \thead{0.31\\(0.66)} & \thead{0.30\\(0.66)} & \thead{0.43\\(0.06)} & \thead{3.27\\(0.53)} & \thead{6.75\\(15.8)} \\ \hline
B & \thead{4578\\(3484)} & \thead{1.28\\(2.05)} & \thead{0.03\\(0.04)} & \thead{0.01\\(0.02)} & \thead{0.26\\(0.03)} & \thead{3.72\\(0.46)} & \thead{1.59\\(2.10)} \\ \hline
\end{tabular}
\end{center}
\caption{Path-tree cost and planning time obtained over 100 planning queries: It indicates the mean value and the standard deviation in parentheses. Planning times are in seconds.}
\label{tab:planning_times}
\end{table}
%%%%
%
In contrast to the examples of the previous section \ref{experiment:navigation}, the planning time is dominated by the random graph creation. This is consistent with the fact that the geometric collision checks are more computationally expensive with this robot. In addition, we note that the planning times have a large dispersion around the mean value (see the standard deviation on \ref{tab:planning_times}), which is due to the higher geometric complexity and dimensionality of the planning problem. Overall, the planning time remains limited to a few seconds.

\subsection{Comparison to baseline} \label{experiment:baseline comparison}
%100 iterations
%advantages: optimality, faster execution times, lightweight setup. No need to bring domain knowledge to set up an action space for a high level search.
We compare PTO to a Task and Motion Planning (TAMP) approach, where the planning is hierarchical: it interleaves a symbolic search defining high level plans, and a motion planning phase computing the corresponding motions. The comparison is performed on variations of the shelf domain (Fig.~\ref{fig:baseline_comparison}), where we plan for the 2D base position only. The number of shelves is varied to compare the scalability.

The high level search is performed using the Branch and Bound algorithm \cite{MORRISON201679}. It explores the space of the possible sequences for visiting all the shelves. The nodes of the search correspond to shelves. The motion planner is queried when a node is created. For each node/shelf, 2 paths are planned using RRT$^{*}$: the path to an observation point, and the path to fetch the object (to be executed if the object is actually detected). A path-tree is obtained by gathering the path pieces from the root node to a leaf of the search tree. 

The branch and bound tree search is performed in a depth-first fashion, which leads to a quick first solution path-tree. The best solution path-tree found so far is an upper bound of the cost and allows the pruning of a majority of the search tree.
We report on Figure \ref{fig:costs_and_runtime} on the average expected cost of the resulting path-trees, as well as on the planning times obtained over 100 planning queries.

%The high-level plans are ordered sequences of shelves to inspect, they are obtained in a breadth-first fashion. For each shelf, 2 paths are planned using RRT$^{*}$: the path to the shelf itself (to pick the object if it is there), and the path towards the next observation point (if the object is not there). The path-tree is obtained by gathering the path pieces planned separately.%

\pgfplotsset{width=5cm, height=7cm}

\begin{figure}[h]  
 \centering
  \begin{subfigure}[t]{0.45\linewidth}
   \center{\includegraphics[width=\textwidth]{drawings/2_arm/baseline_comparison.png}}
   \caption{The green path-tree (PTO) has lower expected cost than the orange path-tree planned with RRT$^{*}$.}
   \label{fig:baseline_comparison}
  \end{subfigure}
  \begin{subfigure}[t]{0.26\linewidth}
    \begin{tikzpicture}[scale=0.55]
	 \begin{axis} [
	    ybar = .05cm,
    	bar width = 3pt,
    	ymin = 0,
    	ymax = 3,
    	xtick = data,
    	enlarge y limits = {value = 0.05, upper},
    	enlarge x limits = {abs = .8},
    	legend pos=north west
		]
		\addplot [green!20!black,fill=green!80!white] coordinates {
		(2, 1.7529471182990233) (4, 2.2212974330517827) (6, 2.3911496782081954) (8, 2.360321441477037)
		};
		\addplot [blue!20!black,fill=blue!80!white] coordinates {
		(2, 1.84) (4, 2.245) (6, 2.441) (8, 2.485)
		};
		\addplot [orange!20!black,fill=orange!80!white] coordinates {
		(2, 1.8569080235157531) (4, 2.3748431227440063) (6, 2.6112924196096783) (8, 2.5971396786963075)
		};
		%\legend {PTO, PRM$^{*}$, RRT$^{*}$}; 
		\end{axis}
	\end{tikzpicture}
    \caption{Path cost (m)}
    \label{fig:cost}
  \end{subfigure}
  \begin{subfigure}[t]{0.26\linewidth}
    \begin{tikzpicture}[scale=0.55]
	 \begin{axis} [ %use /home/camille/Dev/po-rrt/results/map_benchmark/costs_and_timings_with_prm_one.txt
	    ybar = .05cm,
	    ymin = 0.05,
    	bar width = 3pt,
    	ymode=log,
    	log origin=infty,
    	xtick = data,
    	enlarge y limits = {value = .1, upper},
    	enlarge x limits = {abs = .8},
    	legend pos=north west
		]
		\addplot [green!20!black,fill=green!80!white] coordinates {
		(2, 0.0838456953) (4, 0.3447605707) (6, 1.3742766512) (8, 7.585573182200001)
		};
		\addplot [blue!20!black,fill=blue!80!white] coordinates {
		(2, 0.262) (4, 1.674) (6, 6.847) (8, 33.91)
		};
		\addplot [orange!20!black,fill=orange!80!white] coordinates {
		(2, 0.0763110857) (4, 0.8065830762000001) (6, 11.0703240974) (8, 107.3652537214)
		};
		\legend {PTO, PRM$^{*}$, RRT$^{*}$}; 
		\end{axis}
	 \end{tikzpicture}
     \caption{Planning time (s)}
     \label{fig:time}
   \end{subfigure}
   \caption{Comparison of PTO to RRT$^{*}$: \ref{fig:cost} and \ref{fig:time} give the costs and planning times for different number of shelves. PTO provides path-trees with lower costs. Planning time (in log scale) also scales better. }
   \label{fig:costs_and_runtime}
\end{figure}

First, we observe that PTO consistently leads to lower path-tree costs than the piece-wise planning with RRT$^{*}$. This can be understood easily as the decomposition into piecewise motions leads to path pieces that are optimal w.r.t the sub-problem of reaching one shelf, but taken together, they don't form an optimal path-tree. On the other hand, PTO searches for a globally optimal path-tree. It is visible on Fig. \ref{fig:baseline_comparison}: the RRT$^{*}$ path-tree greedily moves towards the next shelf to explore, whereas PTO takes a less direct path to the observation point, which overall leads to a shorter path-tree. 

Second, PTO scales better w.r.t. the number of shelves (see Fig.~\ref{fig:costs_and_runtime}). Planning times are comparable for the variation with 2 shelves, but the difference between PTO and RRT becomes larger when the number of shelves increases. The main reason for this is that PTO is more sample-efficient: The random graph creation (see \ref{section:rapidly-exploring-random-graph}) which involves state and transition checks is constructed just once. On the other hand, the Branch and Bound + RRT$^{*}$ approach is more sample-intensive since a new random tree is re-sampled from scratch for the planning of each path-piece.

In this example, both algorithms PTO and the Branch and Bound search could be made faster by using heuristics as lower bound of the path costs (e.g. euclidean distance). We chose, however, to compare the general approaches, without optimizations tailored to the particular example.  
